Kernel Mean Embedding of Distributions: A Review and Beyond

A Hilbert space embedding of a distribution---in short, a kernel mean embedding---has recently emerged as a powerful tool for machine learning and inference. The basic idea behind this framework is to map distributions into a reproducing kernel Hilbert space (RKHS) in which the whole arsenal of kernel methods can be extended to probability measures. It can be viewed as a generalization of the original "feature map" common to support vector machines (SVMs) and other kernel methods. While initially closely associated with the latter, it has meanwhile found application in fields ranging from kernel machines and probabilistic modeling to statistical inference, causal discovery, and deep learning. The goal of this survey is to give a comprehensive review of existing work and recent advances in this research area, and to discuss the most challenging issues and open problems that could lead to new research directions. The survey begins with a brief introduction to the RKHS and positive definite kernels which forms the backbone of this survey, followed by a thorough discussion of the Hilbert space embedding of marginal distributions, theoretical guarantees, and a review of its applications. The embedding of distributions enables us to apply RKHS methods to probability measures which prompts a wide range of applications such as kernel two-sample testing, independent testing, and learning on distributional data. Next, we discuss the Hilbert space embedding for conditional distributions, give theoretical insights, and review some applications. The conditional mean embedding enables us to perform sum, product, and Bayes' rules---which are ubiquitous in graphical model, probabilistic inference, and reinforcement learning---in a non-parametric way. We then discuss relationships between this framework and other related areas. Lastly, we give some suggestions on future research directions.

==> frontmatter.tex <==
%% Front matter for for FnT Machine Learning
%% (c) 2013 Neal Parikh (Stanford University)
%% 
%% Based on earlier NOW style files by S. Kumar,
%% J. Sebastian, T. Hoekwater, and B.V. Elvenkind
%%
%% Version 1.01 2014-03-19 	No. of Issues in Current 
%% Volume changed to 6.
%% Modified by M. Casey

\RequirePackage{lastpage}
\RequirePackage{multicol}

% base journal information definitions
\def\doi#1{\def\@doi{#1}}
\def\copyrightowner#1{\def\@copyrightowner{#1}}
\def\firstpage#1{\def\@firstpage{#1}}
\def\isbn#1{\def\@isbn{#1}}
\def\issue#1{\def\@issue{#1}}
\def\journalinfofont{\fontsize{8}{10}\selectfont\rmfamily}
\def\journallibraryinfo#1{\def\@libraryinfo{#1}}
\def\journaltitle#1{\def\@journaltitle{#1}}
\def\journaltitleprefix#1{\def\@journaltitleprefix{#1}}
\def\@lastpage{\pageref{LastPage}}
\def\lastpage#1{\def\@lastpage{#1}}
\def\copyrightyear#1{\def\@copyrightyear{#1}}
\edef\@copyrightyear{\the\year}
\def\pubyear#1{\def\@pubyear{#1}}
\edef\@pubyear{\the\year}
\def\volume#1{\def\@volume{#1}}

\def\journaltopicintro#1{\def\@journaltopicintro{#1}}
\def\journaltopics#1{\def\@journaltopics{#1}}

% editors
\newcount\editorcount
\def\@editors{}
\def\journaleditor#1{%
  \advance\editorcount1 
  \ifx\empty\@editors
    \def\@editors{#1}%
  \else
    \expandafter\def\expandafter\@editors\expandafter{\@editors\\[0.3em]#1}%
  \fi
}

% editors in chief
\newcount\chiefeditorcount
\def\@chiefeditors{}
\def\journalchiefeditor#1{%
  \advance\chiefeditorcount1 
  \ifx\empty\@chiefeditors
    \def\@chiefeditors{#1}%
  \else
    \expandafter\def\expandafter\@chiefeditors\expandafter{\@chiefeditors\\[0.3em]#1}%
  \fi
}

%% title page

\renewcommand\maketitle{\begin{titlepage}%

\if@openright % -- for 'book' version
\parindent \z@

% title page
\thispagestyle{empty}
\vspace*{\fill}
\begin{flushright}
\begin{minipage}{0.8\textwidth}
\begin{flushright}
\renewcommand{\baselinestretch}{1.1}
\sffamily\bfseries\huge 
\@title
\end{flushright}
\end{minipage}
\end{flushright}
\vspace*{\fill}

% title+author page
\cleardoublepage
\thispagestyle{empty}

\begin{flushright}
{\renewcommand{\baselinestretch}{1.2}
\sffamily\Huge\bfseries \@title\par}
\vspace{3ex}
\noindent\rule{\textwidth}{2pt}
\vspace{1ex}\par

\begingroup
\def\and{%
  \end{tabular}%
  \par\vspace*{1.5ex}
  \begin{tabular}[t]{r@{}}
  \bfseries}

  \fontsize{13}{15}\selectfont\sffamily
\begin{tabular}[t]{r@{}}
    \bfseries
    \@author
\end{tabular}
\endgroup
\vfill
\includegraphics[width=53bp]{now_logo}\\
\includegraphics[width=81bp]{essence_logo}\\
Boston --- Delft
\end{flushright}

% publisher page
\newpage
\thispagestyle{empty}
\begingroup

\parskip6pt

{\bfseries\sffamily\Large \@journaltitleprefix\ \@journaltitle}
\footnotesize

\vfill

{\itshape Published, sold and distributed by:}\\
now Publishers Inc.\\
PO Box 1024\\
Hanover, MA\ 02339\\
United States\\
Tel.\ +1-781-985-4510\\
www.nowpublishers.com\\
sales@nowpublishers.com

{\itshape Outside North America:}\\
now Publishers Inc.\\
PO Box 179\\
2600 AD Delft\\
The Netherlands\\
Tel.\ +31-6-51115274

The preferred citation for this publication is

%{\raggedright
%\@copyrightowner. \emph{\@title}.  \@journaltitleprefix\
%\@journaltitle, vol.~\@volume, no.~\@issue, pp.~\@firstpage--\@lastpage,
%\@pubyear.\par}

{\itshape This Foundations and Trends\textsuperscript{\textregistered} issue
was typeset in \LaTeX\ using a class file designed by Neal Parikh. Printed on
acid-free paper.}

ISBN: \@isbn\\ \copyright\ \@copyrightyear\ \@copyrightowner

\vfill

\fontsize{8}{9}\selectfont
All rights reserved. No part of this publication may be
reproduced, stored in a retrieval system, or transmitted in any form
or by any means, mechanical, photocopying, recording or otherwise,
without prior written permission of the publishers.

Photocopying. In the USA: This journal is registered at the Copyright
Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923. 
Authorization to photocopy items for
internal or personal use, or the internal or personal use of specific
clients, is granted by now Publishers Inc for users registered with 
the Copyright Clearance Center (CCC).
The `services' for users can be found on the internet at:
www.copyright.com

For those organizations that have been granted a photocopy license, a
separate system of payment has been arranged. Authorization does not
extend to other kinds of copying, such as that for general
distribution, for advertising or promotional purposes, for creating
new collective works, or for resale.  In the rest of the world:
Permission to photocopy must be obtained from the copyright
owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA
02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com;
sales@nowpublishers.com

now Publishers Inc. has an exclusive license to publish this
material worldwide. Permission to use this content must be obtained from
the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
sales@nowpublishers.com\par
\endgroup

% editorial board
\newpage
\thispagestyle{empty}
\begin{center}
\sffamily\LARGE
{\bfseries \@journaltitleprefix\ \@journaltitle}\\
{Volume \@volume, Issue \@issue, \@pubyear}\\
{\bfseries Editorial Board}
\end{center}

\vspace{12pt}

\ifnum\chiefeditorcount>1
{\sffamily\bfseries Editors-in-Chief}
{\footnotesize
\begin{multicols}{2}
\@chiefeditors
\end{multicols}}
\else
{\sffamily\bfseries Editor-in-Chief}\par
\vspace*{10pt}
\begin{footnotesize}
\begin{tabular}[t]{@{}l}
\@chiefeditors \\
\end{tabular}
\end{footnotesize}
\vspace*{10pt}
\fi

{\sffamily \bfseries Editors}
{\footnotesize %\fontsize{9}{11}\selectfont
\begin{multicols}{3}
\raggedcolumns
\@editors
\end{multicols}}%

% editorial scope
\newpage % page vi -- blank
\thispagestyle{empty}
\begin{center}
{\sffamily\bfseries\LARGE Editorial Scope}
\end{center}

\vspace{18pt}

{\bfseries\large\sffamily Topics}\\

\@journaltopicintro

\fontsize{10}{13}\selectfont
\begin{multicols}{2}
    \raggedright
    \@journaltopics
\end{multicols}

{\bfseries\large\sffamily Information for Librarians}\\

\@libraryinfo\par

\else\fi % -- no book front matter for "journal" version

% -- end book front matter

% title+author page
\newpage
\thispagestyle{empty}
\hbox to \textwidth{%
    \vbox{\raggedright
    \hsize=.6\textwidth \journalinfofont
{\hangindent=3.5ex
\hangafter=1
%\@journaltitleprefix\ \@journaltitle\par}%
}
%Vol.~\@volume, No.~\@issue\ (\@pubyear) 
%\@firstpage--\@lastpage\\
%{\hangindent=3.5ex
%\hangafter=1
%\copyright\ \@copyrightyear\ \@copyrightowner\par}%
%DOI: \@doi
}\hss
\vbox{\hsize=.4\textwidth 
    \raggedleft
    %\includegraphics[width=53bp]{now_logo}\\
    %\includegraphics[width=81bp]{essence_logo}\\
    \par
}}\par
\let\footnoterule\relax
\let\footnote\thanks
\null\vfil
\vskip 60\p@
\begin{center}%
{\LARGE \sffamily \bfseries \@title \par}%
\vskip 3em%
{
\large
\lineskip .75em%
     \lineskip .75em%
      \begin{tabular}[t]{c}%
        \@author
      \end{tabular}\par}%
\end{center}\par
\@thanks
\vfill
\end{titlepage}
\setcounter{footnote}{0}%
}

%% defaults and settings for this FnT

\def\@copyrightowner{}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\volume{XX}
\issue{XX}
\firstpage{1}
\isbn{XXX-X-XXXXX-XXX-X}
\doi{10.1561/XXXXXXXXXX}

\journaltitle{Machine Learning}

\journalchiefeditor{\textbf{Michael Jordan} \\
University of California, Berkeley \\
United States}

\journaleditor{Peter Bartlett \\ \emph{UC Berkeley}} 
\journaleditor{Yoshua Bengio \\ \emph{University of Montreal}} 
\journaleditor{Avrim Blum \\ \emph{Carnegie Mellon}} 
\journaleditor{Craig Boutilier \\ \emph{University of Toronto}} 
\journaleditor{Stephen Boyd \\ \emph{Stanford University}} 
\journaleditor{Carla Brodley \\ \emph{Tufts University}} 
\journaleditor{Inderjit Dhillon \\ \emph{UT Austin}} 
\journaleditor{Jerome Friedman \\ \emph{Stanford University}} 
\journaleditor{Kenji Fukumizu \\ \emph{Institute of \\ Statistical Mathematics}} 
\journaleditor{Zoubin Ghahramani \\ \emph{Cambridge University}} 
\journaleditor{David Heckerman \\ \emph{Microsoft Research}} 
\journaleditor{Tom Heskes \\ \emph{Radboud University \\ Nijmegen} \columnbreak} 
\journaleditor{Geoffrey Hinton \\ \emph{University of Toronto}} 
\journaleditor{Aapo Hyvarinen \\ \emph{Helsinki Institute for \\ Information Technology}} 
\journaleditor{Leslie Pack Kaelbling \\ \emph{MIT}} 
\journaleditor{Michael Kearns \\ \emph{University of \\ Pennsylvania}} 
\journaleditor{Daphne Koller \\ \emph{Stanford University}} 
\journaleditor{John Lafferty \\ \emph{Carnegie Mellon}} 
\journaleditor{Michael Littman \\ \emph{Brown University}} 
\journaleditor{Gabor Lugosi \\ \emph{Pompeu Fabra University}} 
\journaleditor{David Madigan \\ \emph{Columbia University}} 
\journaleditor{Pascal Massart \\ \emph{Universit\'e Paris-Sud}} 
\journaleditor{Andrew McCallum \\ \emph{UMass Amherst}} 
\journaleditor{Marina Meila \\ \emph{University of Washington} \columnbreak} 
\journaleditor{Andrew Moore \\ \emph{Carnegie Mellon}} 
\journaleditor{John Platt \\ \emph{Microsoft Research}} 
\journaleditor{Luc de Raedt \\ \emph{University of Freiburg}} 
\journaleditor{Christian Robert \\ \emph{Universit\'e \\ Paris-Dauphine}} 
\journaleditor{Sunita Sarawagi \\ \emph{Indian Institutes \\ of Technology}} 
\journaleditor{Robert Schapire \\ \emph{Princeton University}} 
\journaleditor{Bernhard Schoelkopf \\ \emph{Max Planck Institute}} 
\journaleditor{Richard Sutton \\ \emph{University of Alberta}} 
\journaleditor{Larry Wasserman \\ \emph{Carnegie Mellon}} 
\journaleditor{Bin Yu \\ \emph{UC Berkeley}}

\journaltopicintro{\@journaltitleprefix\ \@journaltitle\ publishes
survey and tutorial articles on the theory, algorithms and applications of machine learning, including the following topics:}

\journaltopics{
\begin{itemize}
\item{Adaptive control and signal processing}
\item{Applications and case studies}
\item{Behavioral, cognitive, and neural learning}
\item{Bayesian learning}
\item{Classification and prediction}
\item{Clustering}
\item{Data mining}
\item{Dimensionality reduction}
\item{Evaluation}
\item{Game theoretic learning}
\item{Graphical models}
\item{Independent component analysis}
\item{Inductive logic programming}
\item{Kernel methods}
\item{Markov chain Monte Carlo}
\item{Model choice}
\item{Nonparametric methods}
\item{Online learning}
\item{Optimization}
\item{Reinforcement learning}
\item{Relational learning}
\item{Robustness}
\item{Spectral methods}
\item{Statistical learning theory}
\item{Variational inference}
\item{Visualization}
\end{itemize}
}

\journallibraryinfo{%
  %Foundations and Trends\textsuperscript{\textregistered} in \@journaltitle, \@pubyear,
  %Volume~\@volume, 6 issues. ISSN paper version 1935-8237.
  %ISSN online version 1935-8245.
  %Also available as a combined paper and online
  %subscription.
}

\endinput

